Anaphoric Binding: an integrated overview

The interpretation of anaphors depends on their antecedents as the semantic value that an anaphor eventually conveys is co-specified by the value of its antecedent. Interestingly, when occurring in a given syntactic position, different anaphors may have different sets of admissible antecedents. Such differences are the basis for the categorization of anaphoric expressions according to their anaphoric capacity, being important to determine what are the sets of admissible antecedents and how to represent and process this anaphoric capacity for each type of anaphor. From an empirical perspective, these constraints stem from what appears as quite cogent generalisations and exhibit a universal character, given their cross linguistic validity. From a conceptual point of view, in turn, the relations among binding constraints involve non-trivial cross symmetry, which lends them a modular nature and provides further strength to the plausibility of their universal character. This kind of anaphoric binding constraints appears thus as a most significant subset of natural language knowledge, usually referred to as binding theory. This paper provides an integrated overview of these constraints holding on the pairing of nominal anaphors with their admissible antecedents that are based on grammatical relations and structure. Along with the increasing interest on neuro-symbolic approaches to natural language, this paper seeks to contribute to revive the interest on this most intriguing research topic.

==> Makefile <==
# specify thh main file and all the files that you are including
SOURCE=  main.tex $(wildcard local*.tex) $(wildcard chapters/*.tex) 

# specify your main target here:
pdf: main.bbl main.pdf  #by the time main.pdf, bib assures there is a newer aux file

all: pod cover

complete: index main.pdf

index:  main.snd
 
main.pdf: main.aux
	xelatex main 

main.aux: $(SOURCE)
	xelatex -no-pdf main 

#create only the book
main.bbl:  $(SOURCE) localbibliography.bib  
	xelatex -no-pdf main 
	biber   main 


main.snd: main.bbl
	touch main.adx main.sdx main.ldx
	sed -i s/.*\\emph.*// main.adx #remove titles which biblatex puts into the name index
	sed -i 's/hyperindexformat{\\\(infn {[0-9]*\)}/\1/' main.sdx # ordering of references to footnotes
	sed -i 's/hyperindexformat{\\\(infn {[0-9]*\)}/\1/' main.adx
	sed -i 's/hyperindexformat{\\\(infn {[0-9]*\)}/\1/' main.ldx
# 	python3 fixindex.py
# 	mv mainmod.adx main.adx
	makeindex -o main.and main.adx
	makeindex -o main.lnd main.ldx
	makeindex -o main.snd main.sdx 
	xelatex main 
 

#create a png of the cover
cover: FORCE
	convert main.pdf\[0\] -quality 100 -background white -alpha remove -bordercolor "#999999" -border 2  cover.png
	cp cover.png googlebooks_frontcover.png
	convert -geometry 50x50% cover.png covertwitter.png
	convert main.pdf\[0\] -quality 100 -background white -alpha remove -bordercolor "#999999" -border 2  -resize x495 coveromp.png
	display cover.png


googlebooks: googlebooks_interior.pdf

googlebooks_interior.pdf: complete
	cp main.pdf googlebooks_interior.pdf
	pdftk main.pdf cat 1 output googlebooks_frontcover.pdf 

openreview: openreview.pdf
	

openreview.pdf: main.pdf
	pdftk main.pdf multistamp orstamp.pdf output openreview.pdf 

proofreading: proofreading.pdf
	
paperhive: 
	git branch gh-pages
	git checkout gh-pages
	git add proofreading.pdf versions.json
	git commit -m 'prepare for proofreading' proofreading.pdf versions.json
	git push origin gh-pages
	git checkout master 
	echo "langsci.github.io/BOOKID"
	firefox https://paperhive.org/documents/new
	
proofreading.pdf: main.pdf
	pdftk main.pdf multistamp prstamp.pdf output proofreading.pdf 

blurb: blurb.html blurb.tex biosketch.tex biosketch.html


blurb.tex: blurb.md
	pandoc -f markdown -t latex blurb.md>blurb.tex
	
blurb.html: blurb.md
	pandoc -f markdown -t html blurb.md>blurb.html
	
biosketch.tex: blurb.md
	pandoc -f markdown -t latex biosketch.md>biosketch.tex
	
biosketch.html: blurb.md
	pandoc -f markdown -t html biosketch.md>biosketch.html
	
#housekeeping	
clean:
	rm -f *.bak *~ *.backup *.tmp \
	*.adx *.and *.idx *.ind *.ldx *.lnd *.sdx *.snd *.rdx *.rnd *.wdx *.wnd \
	*.log *.blg *.ilg \
	*.aux *.toc *.cut *.out *.tpm *.bbl *-blx.bib *_tmp.bib \
	*.glg *.glo *.gls *.wrd *.wdv *.xdv *.mw *.clr \
	*.run.xml \
	chapters/*aux chapters/*~ chapters/*.bak chapters/*.backup\
	langsci/*/*aux langsci/*/*~ langsci/*/*.bak langsci/*/*.backup

realclean: clean
	rm -f *.dvi *.ps *.pdf

chapterlist:
	grep chapter main.toc|sed "s/.*numberline {[0-9]\+}\(.*\).newline.*/\\1/" 

podcover:
	bash podcovers.sh

 

FORCE:


==> langsci/graphics/didyoulikethisbook.tex <==
langsci-advertisement.tex

==> langsci/graphics/langsci-advertisement.tex <==
\thispagestyle{empty}
\pgfdeclarelayer{lspadvert_bg} % Please make sure to never use lspadvert_... PGF layers in any document
\pgfsetlayers{lspadvert_bg,main}

\begin{tikzpicture}[remember picture, overlay,bg/.style={outer sep=0}]
	\begin{pgfonlayer}{lspadvert_bg} % background layer
	\node at (current page.center) [bg, fill=lsGuidelinesGray, minimum height=22cm, minimum width=15cm] (lspadvert_bg1) {}; % Die können wir noch dynamisch bestimmen
	\end{pgfonlayer}	
	\node [execute at begin node={}, font=\fontsize{52pt}{16.75mm}\selectfont, below right = 10mm and 7.5mm of lspadvert_bg1.north west, text width=13.7cm, align=left] (lspadvert_covertitle) {\color{black}\lsCoverTitleFont{Did you like this book?\par}}; % x = 15mm - 7.5mm ; y = 17.5mm - 7.5mm

	\node [font=\fontsize{25pt}{10mm}\selectfont,below = 8mm of lspadvert_covertitle.south, text width=137mm] (lspadvert_coversubtitle) {\color{black} \lsCoverSubTitleFont \nohyphens{This book was brought to you for free}\par}; 
	
	\node (lspadvert_logo) [above left = 10mm and 7.5mm of lspadvert_bg1.south east] {\color{black}\includegraphics{\logopath langsci_logo_nocolor.pdf}};
	\node [above right = 48.8mm and -.1mm of lspadvert_bg1.south west, rectangle, fill=white, minimum size=17pt] (lspadvert_square) {};
	\path let \p1 = (lspadvert_square.north east), \p2 = (lspadvert_covertitle.west) in node at (\x2,\y1) (lspadvert_seriesinfo) [font=\fontsize{17pt}{7.5mm}\selectfont, right, align=flush left, text width=90mm, anchor=north west] {\color{black}\lsCoverSeriesFont{\nohyphens{Please help us in providing free access to linguistic research worldwide. Visit \url{http://www.langsci-press.org/donate} to provide financial support or register as a community proofreader or typesetter \mbox{at \url{http://www.langsci-press.org/register}.}}\par}};
\end{tikzpicture} 

==> langsci/seriesinfo/algad-info.tex <==
%% -*- coding:utf-8 -*-
{\large African Language Grammars and Dictionaries}

\bigskip

Chief Editor:    Adams Bodomo \\
Editors:    Ken Hiraiwa,    Firmin Ahoua 

\bigskip

In this series:

\begin{enumerate}
\item Brindle, Jonathan. A dictionary and grammatical outline of Chakali
\item Friesen, Dianne. A grammar of Moloko.
\end{enumerate}


\vfill

% \gdef\lsISSN{XXXX-YYYY}%
% \hfill ISSN: \lsISSN


==> langsci/seriesinfo/calseries-info.tex <==
%% -*- coding:utf-8 -*-
{\large African Language Grammars and Dictionaries}

\bigskip

Editors:  Lee Bickmore,  Akinbiyi Akinlabi 


\bigskip

In this series:

\begin{enumerate}
\item Payne, Doris L., Sara Pacchiarotti \& Mokaya Bosire (eds.). Diversity in African languages: Selected papers from the 46th Annual Conference on African Linguistics.
\end{enumerate}


\vfill

% \gdef\lsISSN{XXXX-YYYY}%
% \hfill ISSN: \lsISSN


==> langsci/seriesinfo/cfls-info.tex <==
%% -*- coding:utf-8 -*-
{\large Conceptual Foundations of Language Science}

\bigskip

\textbf{Series editors}\\
Mark Dingemanse, \textit{Max Planck Institute for Psycholinguistics}   \\
N. J. Enfield, \textit{University of Sydney}


\bigskip


\textbf{Editorial board}\\
Balthasar Bickel, \textit{University of Zürich},    
Claire Bowern, \textit{Yale University},           
Elizabeth Couper-Kuhlen, \textit{University of Helsinki},     
William Croft, \textit{University of New Mexico},             
Rose-Marie Déchaine, \textit{University of British Columbia},       
William A. Foley, \textit{University of Sydney} ,                   
William F. Hanks, \textit{University of California at Berkeley},    
Paul Kockelman, \textit{Yale University},            
Keren Rice, \textit{University of Toronto},          
Sharon Rose, \textit{University of California at San Diego},        
Frederick J. Newmeyer, \textit{University of Washington},         
Wendy Sandler, \textit{University of Haifa},             
Dan Sperber \textit{Central European University}


\bigskip
\bigskip

\begin{minipage}{\textwidth}% for undoing \raggedright and justify the following two paragraphs

No scientific work proceeds without conceptual foundations. In language science, our concepts about language determine our assumptions, direct our attention, and guide our hypotheses and our reasoning. Only with clarity about conceptual foundations can we pose coherent research questions, design critical experiments, and collect crucial data. 
%
This series publishes short and accessible books that explore well-defined topics in the conceptual foundations of language science. The series provides a venue for conceptual arguments and explorations that do not require the traditional book-length treatment, yet that demand more space than a typical journal article allows.  
\end{minipage}

\bigskip
\bigskip

In this series:

\begin{enumerate}
\item N. J. Enfield. \textit{Natural causes of language}.

\end{enumerate}




==> langsci/seriesinfo/classics-info.tex <==
%% -*- coding:utf-8 -*-
{\large Classics in Linguistics}

\bigskip

Chief Editors: Martin Haspelmath, Stefan Müller

\bigskip

In this series:

\begin{enumerate}
\item Lehmann, Christian. Thoughts on grammaticalization.
\item Schütze, Carson T. The empirical base of linguistics: Grammaticality judgments and linguistic methodology.
\item Bickerton, Derek. Roots of language.
\item von der Gabelentz, Georg. Die Sprachwissenschaft:  Ihre Aufgaben, Methoden und bisherigen Ergebnisse. 
\end{enumerate}


\vfill

% \gdef\lsISSN{XXXX-YYYY}%
% \hfill ISSN: \lsISSN


==> langsci/seriesinfo/cmle-info.tex <==
%% -*- coding:utf-8 -*-
{\large Computational Models of Language Evolution}

\bigskip

Editors: Luc Steels, Remi van Trijp

\bigskip

In this series:

\begin{enumerate}
\item Steels, Luc. The Talking Heads Experiment: Origins of words and meanings.
\item Vogt, Paul. How mobile robots can self-organize a vocabulary.
\item Bleys, Joris. Language strategies for the domain of colour.
\item van Trijp, Remi. The evolution of case grammar.
\item Spranger, Michael. The evolution of grounded spatial language.
\end{enumerate}




==> langsci/seriesinfo/eotms-info.tex <==
%% -*- coding:utf-8 -*-
{\large Em­pir­i­cal­ly Ori­ent­ed The­o­ret­i­cal Mor­phol­o­gy and Syn­tax}

\bigskip

Chief Editor: Stefan Müller  \\
Consulting Editors: Berthold Crysmann, Laura Kallmeyer

\bigskip

In this series:

\begin{enumerate}
\item Lichte, Timm. Syntax und Valenz: Zur Modellierung kohärenter und elliptischer Strukturen mit Baumadjunktionsgrammatiken
%\item  Bîlbîie, Gabriela. Grammaire des constructions elliptiques: Une étude comparative des phrases sans verbe en roumain et en français 
\end{enumerate}





==> langsci/seriesinfo/lv-info.tex <==
%% -*- coding:utf-8 -*-
{\large Language Variation}

\bigskip

Editors: John Nerbonne, Dirk Geeraerts

\bigskip

In this series:

\begin{enumerate}
\item Côté, Marie-Hélène, Remco Knooihuizen and John Nerbonne (eds.). The future of dialects.
\item Schäfer, Lea. 2016. Sprachliche Imitation: Jiddisch in der deutschsprachigen
Literatur (18.–20. Jahrhundert).
Press.
\end{enumerate}



\vfill

% \gdef\lsISSN{XXXX-YYYY}%
% \hfill ISSN: \lsISSN




==> langsci/seriesinfo/sidl-info.tex <==
%% -*- coding:utf-8 -*-
{\large Studies in Diversity Linguistics}

\bigskip

Chief Editor: Martin Haspelmath \\
Consulting Editors: Fernando Zúñiga, Peter Arkadiev, Ruth Singer, Pilar Valen­zuela

\bigskip

In this series:

\begin{enumerate}
\item Handschuh, Corinna. A typology of marked-S languages.
\item Rießler, Michael. Adjective attribution.
\item Klamer, Marian (ed.). The Alor-Pantar languages: History and typology.
\item Berghäll, Liisa. A grammar of Mauwake (Papua New Guinea).
\item Wilbur, Joshua. A grammar of Pite Saami.
\item Dahl, Östen. Grammaticalization in the North: Noun phrase morphosyntax in Scandinavian vernaculars.
\item Schackow, Diana.    A grammar of Yakkha.
\item Liljegren, Henrik. A grammar of Palula.
\item Shimelman, Aviva. A grammar of Yauyos Quechua. 
\item Rudin, Catherine \& Bryan James Gordon (eds.). Advances in the study of Siouan languages and linguistics.
\item Kluge, Angela. A grammar of Papuan Malay. 
\item Kieviet, Paulus. A grammar of Rapa Nui. 
\item Michaud, Alexis. Tone in Yongning Na: Lexical tones and morphotonology.
\item Enfield, N.\,J (ed.).  Dependencies in language: On the causal ontology of linguistic systems .
\item Gutman, Ariel. Attributive constructions in North-Eastern Neo-Aramaic.
\item Bisang, Walter \& Andrej Malchukov (eds.). Unity and diversity in grammaticalization scenarios.
 
\end{enumerate}





==> langsci/seriesinfo/silp-info.tex <==
%% -*- coding:utf-8 -*-

{\raggedleft\IfFileExists{./langsci/seriesinfo/labphon-logo.pdf}{\includegraphics[width=5cm]{./langsci/seriesinfo/labphon-logo.pdf}}{LabPhon-Logo}}

\bigskip

{\large Studies in Laboratory Phonology}

\bigskip

Chief Editor:  Martine Grice% (Chief Editor, University of Cologne, Germany),
\\
Editors:    Doris Mücke, % (University of Cologne, Germany),
    Taehong Cho % (Hanyang University, Seoul, South Korea)

\bigskip

In this series:

\begin{enumerate}
\item Cangemi, Francesco. Prosodic detail in Neapolitan Italian.
\item Drager, Katie. linguistic variation, identity construction, and cognition.
\end{enumerate}








==> langsci/seriesinfo/tbls-info.tex <==
%% -*- coding:utf-8 -*-
{\large Textbooks in Language Sciences}

\bigskip

Editors: Stefan Müller, Martin Haspelmath  \\
Editorial Board: Claude Hagège, Marianne Mithun, Anatol Stefanowitsch, Foong Ha Yap

\bigskip

In this series:

\begin{enumerate}
\item Müller, Stefan. Grammatical theory: From transformational grammar to constraint-based approaches.
\item Schäfer, Roland. Einführung in die grammatische Beschreibung des Deutschen.
\end{enumerate}





==> langsci/seriesinfo/tmnlp-info.tex <==
%% -*- coding:utf-8 -*-
{\large Translation and Multilingual Natural Language Processing}

\bigskip

Editors: Oliver \v{C}ulo (Johannes Gutenberg-Universität Mainz),
Silvia Hansen-Schirra (Johannes Gutenberg-Universität Mainz), 
Stella Neumann (RWTH Aachen),
Reinhard Rapp (Johannes Gutenberg-Universität Mainz)

\bigskip

In this series:

\begin{enumerate}
\item Fantinuoli, Claudio \& Federico Zanettin (eds.). New directions in corpus-based translation studies.
\item Hansen-Schirra, Silvia \& Sambor Grucza (eds.). Eyetracking and Applied Linguistics.
\item Neumann, Stella, Oliver Čulo \& Silvia Hansen-Schirra (eds.). Annotation, exploitation and evaluation of parallel corpora: TC3\,I.
\item Čulo, Oliver  \& Silvia Hansen-Schirra (eds.). Crossroads between Contrastive Linguistics, Translation Studies and Machine Translation: TC3\,II.
\item Rehm, Georg, Felix Sasaki, Daniel Stein \& Andreas Witt (eds.). Language technologies for a multilingual Europe: TC3\,III.
\item Menzel, Katrin, Ekaterina Lapshinova-Koltunski \& Kerstin Anna Kunz  (eds.). New perspectives on cohesion and coherence: Implications for translation.
\end{enumerate}

 


==> localseealso.tex <==
\is{some term| see {some other term}}
\il{some language| see {some other language}}
\issa{some term with pages}{some other term also of interest}
\ilsa{some language with pages}{some other lect also of interest}
